eXpath: Explaining Knowledge Graph Link Prediction with Ontological Closed Path Rules

Link prediction (LP) is crucial for Knowledge Graphs (KG) completion but commonly suffers from interpretability issues. While several methods have been proposed to explain embedding-based LP models, they are generally limited to local explanations on KG and are deficient in providing human interpretable semantics. Based on real-world observations of the characteristics of KGs from multiple domains, we propose to explain LP models in KG with path-based explanations. An integrated framework, namely eXpath, is introduced which incorporates the concept of relation path with ontological closed path rules to enhance both the efficiency and effectiveness of LP interpretation. Notably, the eXpath explanations can be fused with other single-link explanation approaches to achieve a better overall solution. Extensive experiments across benchmark datasets and LP models demonstrate that introducing eXpath can boost the quality of resulting explanations by about 20% on two key metrics and reduce the required explanation time by 61.4%, in comparison to the best existing method. Case studies further highlight eXpath's ability to provide more semantically meaningful explanations through path-based evidence.

==> backup/tex/1_intro.tex <==
\section{Introduction}

Knowledge graphs (KGs) commonly suffer from incompleteness, leading to the development of various methods for knowledge graph completion (KGC). Link prediction (LP) is a crucial task in KGC, aiming to predict potential missing relationships between entities within a KG. Among these methods, knowledge graph embedding (KGE) models have become dominant, mapping entities and relationships into continuous vector spaces to infer missing information. Advanced KGE models such as ComplEx~\cite{trouillon2016complex}, TransE~\cite{wang2014knowledge}, DistMult~\cite{yang2014embedding}, and ConvE~\cite{dettmers2018convolutional} have been applied to mainstream KGs like Freebase~\cite{bollacker2008freebase}, DBpedia~\cite{auer2007dbpedia}, and YAGO~\cite{mahdisoltani2014yago3} to deduce absent links, surpassing traditional rule-based systems. However, despite their effectiveness, these models often function as black boxes, hindering interpretability. The field of eXplainable AI (XAI) has emerged to address this challenge, aiming to explain the behavior and predictions of KGE models. The need for interpretability is particularly urgent in applications where high-stakes decisions are made based on model predictions. For example, in financial networks, link prediction can be used to detect potential fraud or credit risks. 

In response to this need for interpretability, various methods have been developed to understand the behavior of Link Prediction models. These include approaches for explaining GNN-based LP model~\cite{ying2019gnnexplainer, zhang2023page, chang2024path} embedding-based LP model~\cite{bhardwaj2021adversarial, zhang2019data},
providing fact-based, path-based, rule-based~\cite{meilicke2024anytime, betz2022adversarial}, or subgraph-based explanations~\cite{yuan2021explainability, zhang2022gstarx, zhao2023ke}. Among these, adversarial attack methods~\cite{bhardwaj2021adversarial, pezeshkpour2019investigating} become prominent. These methods propose minimal modifications to a knowledge graph, aiming to have a maximal negative effect on the prediction of a correct prediction. For example, kelpie~\cite{rossi2022explaining}captures the model's sensitivity to fact removal and addition by utilizing entity mimic and post-training techniques. However, these approaches are limited in two key ways. First, they only provide local explanations, focusing on the properties of the head or tail entity, without considering the full path. Second, they often lack semantic clarity, which undermines their trustworthiness, even though they are effective at predicting the correct outcomes.


\begin{figure}[t]
\vspace{-1cm}
\includegraphics[width=\columnwidth]{pic/MOFexampleV3.png}
\vspace{-0.5cm}
\caption{A clip of the materials synthesis KG. To explain the prediction ⟨BEMHUX (a material), hasSolvent, dichloromethane (a solvent)⟩ by LP models, two key paths are identified: BEMHUX and dichloromethane share the same structure, and BEMHUX appears in the same paper as another material, BEMHIL, which also uses dichloromethane as a solvent. Fact-based explanation methods (e.g., Kelpie) provide the bolded facts as explanations, but they lack interpretable semantics without paths connecting them.} 
\label{MOFexample}
\vspace{-0.4cm}
\end{figure}

Through our observations, we find that certain knowledge graphs exhibit recurring patterns that can enhance the interpretability of predictions. For instance, in material knowledge graphs (Fig.~\ref{MOFexample}), a task like predicting solvents can be better explained by considering the relationship paths between materials and solvents, rather than focusing solely on the properties of individual entities, as identified by Kelpie~\cite{rossi2022explaining}. In such cases, path-based explanations, such as the 2-hop and 3-hop paths, provide richer and more comprehensible insights. The 2-hop path reflects a shared structure between materials and solvents, while the 3-hop path indicates that a solvent appears in a paper with another material, establishing an analogy. In synthesis tasks and similar scenarios, path-based explanations can significantly improve the interpretability of predictions.

Building on this observation, we propose a path-based explanation approach that not only suggests minimal modifications but also provides semantically meaningful paths that support each modification. However, addressing this problem presents several challenges. First, there is the issue of scalability: given that each prediction may involve thousands of potential paths, selecting the most relevant ones is computationally expensive. Second, evaluating the impact of these paths on embedding models is challenging because the paths alter the dataset in a way that is more significant than the localized modifications typically used in traditional adversarial attacks.

To address these challenges, we introduce relation path aggregation and a post-training pruning method to effectively reduce the number of paths considered. Then we draw on ontological rules and propose a fact-scoring method to evaluate the relevance of paths, allowing us to select the most meaningful explanations based on these rules. Our primary contributions are as follows:

\begin{itemize}
  \item Define the path-based explanation problem and integrate semantically rich ontological rules into the adversarial attack framework.
  \item Propose a comprehensive methodology, including relation path aggregation, rule mining with post-training pruning, and explanation construction through fact scoring.
  \item Conduct extensive experiments across multiple models and datasets, demonstrating that our method not only identifies influential triples but also provides clear path-based explanations of underlying statistical patterns.
\end{itemize}

==> backup/tex/2_related.tex <==
\section{Related Work}

\subsection{Knowledge Graph Link Prediction (KGLP) Explainability}

Explainability in Knowledge Graph Link Prediction (KGLP) is a critical area of research due to the increasing complexity of models used in link prediction tasks. General-purpose explainability techniques are widely used to understand the input features most responsible for a prediction. LIME~\cite{ribeiro2016should} creates local, interpretable models by perturbing input features and fitting regression models, while SHAP~\cite{lundberg2017unified} assigns feature importance scores using Shapley values from game theory. ANCHOR~\cite{ribeiro2018anchors} identifies "anchors," consistent feature sets that ensure reliable predictions across samples.  These frameworks have been widely adopted in various domains, including adaptations for graph-based tasks, although their application in link prediction for knowledge graphs remains limited.

GNN-based LP explainability primarily focuses on interpreting the internal workings of Graph Neural Networks (GNNs)-based link prediction models. Techniques like GNNExplainer~\cite{ying2019gnnexplainer} and PGExplainer~\cite{luo2020parameterized} identify influential subgraphs through mutual information, providing insights into node and graph-level predictions, although they are not directly applicable to link prediction tasks. Other methods, such as SubgraphX~\cite{yuan2021explainability} and GStarX~\cite{zhang2022gstarx}, use game theory values to select subgraphs relevant to link prediction, while PaGE-Link~\cite{zhang2023page} argues that paths are more interpretable than subgraphs and extends the explanation task to the link prediction problem on heterogeneous graphs. Additionally, Power-Link~\cite{chang2024path}, a path-based KGC explainer, leverages a graph-powering technique for more memory-efficient and parallelizable explanations. However, GNN-based explainability techniques are limited to GNN-based LP models and do not extend to Embedding-based approaches.

\subsection{Embedding-based LP Explainability}

Embedding-based LP explainability is more versatile than GNN-based LP explainability, as it is not restricted to GNN-based models and is primarily focused on providing local post-hoc explanations and assessing the robustness of Knowledge Graph Embedding (KGE) models. These methods are categorized into white-box and black-box approaches.

White-box methods propose algorithms that approximate the impact of graph modifications on specific predictions and identify crucial changes. Criage~\cite{pezeshkpour2019investigating} applies first-order Taylor approximations for estimating the impact of removing facts on prediction scores. Data Poisoning~\cite{bhardwaj2021adversarial, zhang2019data} manipulates embeddings by perturbing entity vectors to degrade the model’s scoring function, highlighting pivotal facts during training. ExamplE~\cite{janik2022explaining} introduce ExamplE heuristics, which generate disconnected triplets as influential examples in latent space. KE-X~\cite{zhao2023ke} leverages information entropy to quantify the importance of explanation candidates and explains KGE-based models by extracting valuable subgraphs through a modified message-passing mechanism. While these white-box methods offer valuable insights, they often require full access to model parameters, making them impractical for real-world applications.

Recent research has also focused on black-box adversarial attacks, which do not require knowledge of the underlying model architecture. KGEAttack~\cite{betz2022adversarial} uses rule learning and abductive reasoning to identify critical triples influencing predictions, offering a model-agnostic alternative to white-box methods. Kelpie~\cite{rossi2022explaining} explains KGE-based predictions by identifying influential training facts, utilizing mimic and post-training techniques to sense the underlying embedding mechanism without relying on model structure. However, these methods are typically limited to explaining fact-based relationships and fail to capture the multi-relational context that is crucial for full interpretability in knowledge graphs.


\subsection{Ontological Rules for Knowledge Graph}

Ontological rules for knowledge graphs have been a prominent area of research, as they provide symbolic and interpretable reasoning over knowledge graph data. Early work such as AMIE~\cite{galarraga2013amie, galarraga2015fast} and AnyBURL~\cite{meilicke2020reinforced, meilicke2024anytime} focused on leveraging Horn rules to infer missing facts in knowledge graphs, providing human-understandable explanations. These methods extract rules from large RDF knowledge bases and use efficient pruning techniques to generate high-quality rules with minimal parameter tuning. Path-based rule learning has also been explored to improve link prediction explainability. Bhowmik~\cite{bhowmik2020explainable} proposes a framework emphasizing reasoning paths to improve link prediction interpretability in evolving knowledge graphs. RLvLR~\cite{omran2018scalable, omran2019embedding} combines embedding techniques with efficient sampling to optimize rule learning for large-scale and streaming KGs. While these methods excel in structural reasoning, they are limited in directly explaining predictions made by embedding-based models, highlighting a gap in integrating rule-based reasoning with KGE interpretability.

Recent works have explored the use of ontological rules to explain embedding-based models. Several studies have sought to combine symbolic reasoning with KGE models. For instance, Guo et al.~\cite{guo2018knowledge} introduced rules as background knowledge to enhance the training of embedding models, while Zhang et al.~\cite{zhang2019iteratively} proposed an alternating training scheme that incorporates symbolic rules. These approaches aim to bridge the gap between symbolic reasoning and KGE performance. A more recent study by Meilicke et al.~\cite{meilicke2021naive} demonstrated that symbolic and sub-symbolic models share commonalities, suggesting that KGE models may indeed be explained using rule-based approaches. This insight underpins the notion that embedding models and ontological rules can complement each other to provide a richer, more interpretable explanation for link prediction tasks.




==> backup/tex/3_background.tex <==
\section{Background and problem definition}
\subsection{KGLP Explanation}

Knowledge Graphs (KGs), denoted as $KG = (\mathcal{E}, \mathcal{R}, \mathcal{G})$, are structured representations of real-world facts, where entities from $\mathcal{E}$ are connected by directed edges in $\mathcal{G}$, each representing semantic relations from $\mathcal{R}$. These edges represent facts of the form $f = ⟨h, r, t⟩$, where $h$ is the head entity, $r$ is the relation, and $t$ is the tail entity. Link Prediction (LP) aims to predict missing relations between entities in a KG. The standard approach to LP is embedding-based, where entities and relations are embedded into continuous vector spaces, and a scoring function, $f_r(h,t)$, is used to measure the plausibility of a fact. Evaluation of LP models is typically performed using metrics such as mean reciprocal rank (MRR), which measures how well the model ranks the correct entities when predicting missing heads or tails in test facts.

\[
MRR = \frac{1}{2|\mathcal{G}_e|} \sum_{f \in \mathcal{G}_e} \left( \frac{1}{\operatorname{rk}_h(f)} + \frac{1}{\operatorname{rk}_t(f)} \right)
\]

Where $\operatorname{rk}_t(f)$ represents the rank of the target candidate $t$ in the query $⟨h, r, ?⟩$, and $\operatorname{rk}_h(f)$ the rank of the target candidate $h$ in the query $⟨?, r, t⟩$. While embedding-based LP provides accurate predictions, understanding the reasoning behind these predictions is crucial for model transparency and trust. To address this, explanations for embedding-based LP are explored.

Embedding-based LP explanations focus on providing local instance-level explanations for individual predictions. These explanations aim to uncover the underlying features of the embeddings—such as proximity, shared neighbors, or similar latent factors—that contribute to the predicted link. The goal is to understand why a specific prediction is made, enhancing transparency and trust in the model.

However, these explanation methods do not directly perturb the model's architecture or the embeddings themselves. Instead, they rely on adversarial perturbations in the training data. We explore both adversarial additions and adversarial deletions, where the attacker is restricted to making small edits within the neighborhood of the target triple. These perturbations help assess the robustness of Knowledge Graph Embedding (KGE) models and provide insights into the factors influencing link predictions.

\subsection{Adversarial Attack Problem}

Adversarial attacks in the context of KGLP explanations are designed to evaluate the stability of link prediction models by intentionally degrading their performance through targeted perturbations in the training data. These attacks help to reveal how vulnerable a model is to small changes in the graph and, by extension, provide insights into the model's robustness.

Adversarial attacks provide instance-level adversarial modifications as explanations. Given a prediction $⟨h,r,t⟩$, an explanation can be seen as the smallest set of training facts that enabled the model to predict either the tail $t$ in $⟨h, r, t⟩$ or the head $h$ in $⟨h, r, ?⟩$. For example, to explain why the top-ranked tail for $⟨Barack\_Obama, nationality, ?⟩$ is USA, we search for the smallest set of facts whose removal from the training set $\mathcal{G}_{\text{train}}$ would lead the model to change its prediction for $⟨h, r, ?⟩$ from USA to any entity $e \neq t$, and for $⟨?, r, t⟩$ from $h$ to any entity $e' \neq h$. These facts can involve not only the head entity but also the tail entity, as they play an important role in the prediction.

We evaluate the impact of the adversarial attack by comparing standard metrics, such as MRR, before and after the attack. Specifically, we train the model on the original training set and select a small subset of the test set $T \subset \mathcal{G}_e$ as target triples for which the model achieves good predictive performance. After removing the attack set from the training set, we retrain the model and measure the degradation in performance on the target set.

Since we focus on small perturbations, the attack is restricted to deleting a small set of triples. To make this process computationally feasible, we adopt a batch mode where the deletion of one target triple may affect others. If the target sets are small and the predicates contain disjoint entities, dependencies between triples are rare and can typically be neglected. The explanatory capability of the attack is measured by the degradation in MRR, defined as:

\[
\delta MRR(T) = 1 - \frac{MRR_{\text{new}}(T)}{MRR_{\text{original}}(T)}
\]

\subsection{Path-Based Adversarial Attack Problem}

While adversarial attacks focus on generating explanations for individual predictions, they often lack a clear rationale or justification for why certain facts are considered critical. We observe that certain knowledge graphs exhibit recurring patterns that can enhance the interpretability of predictions. In particular, facts that form part of a path connecting the head and tail entities are often crucial because they provide a structural rationale for the prediction. Understanding these critical paths can enrich the explanation and highlight the importance of recurring facts across multiple paths.

In this work, we define the Path-Based Adversarial Attack Problem. Given a prediction $⟨h,r,t⟩$, an explanation consists of the smallest set of training facts that enable us to make the prediction. Additionally, we provide the rationale for each fact's inclusion in the explanation, specifically that it exists within one or more critical paths. A critical path is defined as an important relation path from the head to the tail entity: $\langle h, r_1, A_1 \rangle \land \langle A_1, r_2, A_2 \rangle \land \dots \land \langle A_{n-1}, r_n, t \rangle$, where \( h \) and \( t \) represent the head and tail entities, \( r_i \) denotes relations, and \( A_i \) represents any intermediate entity (denoted in uppercase as a placeholder, not a specific entity). This sequence of triples forms a path from the head to the tail entities. Each critical path corresponds to a high-confidence ontological rule that supports the prediction.

Path-based explanations focus on tracing these facts and associating facts with paths. However, several challenges arise when dealing with such paths:  
\begin{itemize}
    \item Explosive Path Combinatorics: The number of paths between a head and a tail can be vast, especially in large datasets like FB15k-237, where an average of 7,242 paths exists between entities. Exhaustively searching such a large space is computationally impractical.  
    \item Evaluating Path Impact: Evaluating the impact of these paths on embedding models is more complex than traditional adversarial attacks, as paths alter the dataset in a way that is more significant than localized changes.  
    \item Multi-Path Fact Importance: A single fact may participate in many paths and play crucial roles in different contexts. As explanations are constrained to a fixed set of facts, determining the relative importance of each fact across these paths becomes essential.
\end{itemize}

It is important to distinguish our path-based adversarial attack approach from related methods such as Power-Link~\cite{chang2024path}. Unlike Power-Link, which uses multiple simple paths for explanation sets, we demonstrate that using simple paths in embedding-based LP scenarios may not be as effective. Instead, we rely on special ontological rule-based relation paths. Furthermore, while other adversarial methods focus purely on facts, our explanations also consider critical paths that highlight the importance of certain facts, providing a richer, more interpretable rationale. We will demonstrate the efficacy and comprehensibility of this approach in our case study.


==> backup/tex/4_framework.tex <==
\section{eXpath Method}

The eXpath method is designed to provide explanations for any given prediction $⟨h, r, t⟩$ by identifying a small yet effective set of triples whose removal significantly impacts the model's predicted ranking of $h$ and $t$. This process highlights the importance of those facts in contributing to the prediction. Additionally, eXpath provides the rationale for its explanations by presenting the set of paths associated with each selected fact.

The core ideology of eXpath lies in the observation that facts within an explanation set are often critical because they play essential roles in one or more paths that support a prediction. To implement this, eXpath evaluates the contribution of each fact by considering all the paths it satisfies and assigning scores based on aggregated importance across these paths (discussed in detail in Section 4.3). This scoring system enables the framework to prioritize facts that have a significant impact on the model’s prediction.

A crucial step in this process is constructing a path set $\Phi$, which is computed for each prediction within a small, localized graph relevant to that prediction. However, the potentially vast search space for paths, especially when considering paths longer than 3, poses a significant computational challenge. To address this, eXpath aggregates these paths into abstract relation paths and incorporates two types of rules borrowed from Ontological Rule Learning: close-path rules (CP) and Property transition (PT), which will be detailed in Section 4.1.

To effectively mine and evaluate these rules, eXpath first employs a local optimization method to filter CP rules. Subsequently, it uses a matrix-based approach to efficiently evaluate the validity and significance of these rules (discussed in Section 4.2).


\subsection{Relation Path and Rule}

\begin{figure}[t]
\includegraphics[width=\columnwidth, clip, trim=5pt 5pt 5pt 5pt]{pic/ruleExampleV5.png}
\caption{Principles and instances of ontological rules used in our framework. Close-path (CP) rules describe the relationship between entities \(X\) and \(Y\) through alternative paths, while Property Transition (PT) rules capture transitions between different attributes of the same entity. These ontological rules are not predefined but are generalized patterns mined from the knowledge graph, supported by substructures that conform to the specified patterns.}
\label{ruleExample}
\end{figure}

To support path-based explanations, we employ BFS to search for paths between the head and tail entities. However, the number of such paths grows exponentially with the path length, making even 3-hop paths computationally prohibitive. To mitigate this issue, we focus not on the specific entities traversed by a path but rather on the sequence of relations along the path. This abstraction, referred to as a "relation path," drastically reduces the number of candidate paths while preserving their semantic meaning. This concept is inspired by the use of \textit{close-path rules} (CP) in ontological rule learning. By aggregating multiple simple paths into relation paths, we achieve a significant reduction in path count, while retaining the interpretability crucial for explanations. CP rules describe the relationship between entities \(X\) and \(Y\) via alternative paths, which may consist of one or more relations without considering intermediate entities. Additionally, these relations can include recursive rules (i.e., relations that cycle back to the same predicate).

Figure~\ref{ruleExample} illustrates examples of CP rules and PT rules, which are defined as binary rules and unary rules with an atom that ends with a constant in ontological rule mining. While PT rules can be generalized into CP rules by adding relationships between constants and replacing constants with variables, they remain essential for scenarios where two constant entities are strongly correlated (e.g., \texttt{male} and \texttt{female}) but cannot be described by simple paths. These interpretable rules offer clear insights into link predictions, providing a strong foundation for generating explanations. Formally, we distinguish between two types of rules:
\begin{equation}
\label{eq:rule}
\begin{aligned}
\mathbf{CP}: & \quad r\left(A_0, A_n\right) \leftarrow \bigwedge_{i=1}^n r_i\left(A_{i-1}, A_i\right) \\
\mathbf{PT}: & \quad r\left(X, c\right) \leftarrow r'\left(X, c^{\prime}\right)\quad \text{or} \quad r\left(c, Y\right) \leftarrow r'\left(c^{\prime}, Y\right)
\end{aligned}
\end{equation}
Here, \(r\) and \(r_i\) denote relations (binary predicates), \(A_0, A_i, A_n, X, Y\) are variables, and \(c, c^{\prime}\) are constants (entities). We use \(\phi\) to denote a rule, where the atoms on the left (\(h\)) form the \textit{head} of the rule (\(head(\phi)\)), and the atoms on the right (\(r\)) form the \textit{body} of the rule (\(body(\phi)\)). To simplify the notation, in the following part, we use $h\leftarrow r_1,r_2,...,r_n$ to symbolize CP rules, and relations can be reversed to capture inverse semantics (noted with a overline symbol, \(\overline{r}\)). For example, the relation \texttt{hypernym(X, Y)} can also be expressed as \texttt{hypernym'(Y, X)}.

CP rules are termed "closed paths" because the sequence of predicates in the rule body forms a path that directly connects the subject and object arguments of the head predicate. This characteristic establishes a strong connection between CP rules and relation paths. Both concepts focus on capturing the structured relationships between entities in a knowledge graph, and their forms are inherently aligned. This alignment allows relation paths to serve as direct candidates for CP rule bodies. In fact, every CP rule can be viewed as a formalized and generalized representation of a relation path, enriched with additional semantic information, such as confidence and support.  Moreover, the structured nature of CP rules makes them well-suited for explaining embedding-based predictions, as they encapsulate the critical relational patterns that underpin the model's reasoning.

To assess the quality of rules, we recall measures used in some major approaches to rule learning~\cite{chen2016scalekb}~\cite{galarraga2015fast}. Let $\phi$ be a CP rule of the form ~\ref{eq:rule}. A pair of entities $r\left(e, e'\right)$ satisfies the head of $\phi$ and there exist entities $e_1, \ldots, e_{n-1}$ in the KG such that $⟨e,r_1,e_1⟩, \ldots, ⟨e_{n-1},r_n,e'⟩$ are facts in the KG, so the body of $R$ are satisfied. Then the support degree of $\phi$ is defined as

$$
\operatorname{supp}(\phi)=\#\left(e, e^{\prime}\right): \operatorname{body}(\phi)\left(e, e^{\prime}\right) \wedge r\left(e, e^{\prime}\right)
$$


To normalize this degree, the degrees of standard confidence (SC) and head coverage ( HC ) are defined as follows:

$$
S C(\phi)=\frac{\operatorname{supp}(\phi)}{\#\left(e, e^{\prime}\right): \operatorname{body}(\phi)\left(e, e^{\prime}\right)}, H C(r)=\frac{\operatorname{supp}(\phi)}{\#(e, e): P_t\left(e, e^{\prime}\right)}
$$

\begin{figure*}[t]
\includegraphics[width=\textwidth]{pic/pipelineV4.png}
\caption{Pipeline of rule mining for CP rules related to the prediction. (a) \textit{Path Exploring}: searching for paths between the head and tail entities using BFS and condensing them into relation paths; (b) \textit{Rule Filtering}: using a local optimization method to identify candidate rules; (c) \textit{Rule Evaluation}: assessing the significance of candidate rules through a matrix-based approach.}
\label{rulemining}
\end{figure*}

\subsection{Rule Mining}

\begin{algorithm}[!h]
    \caption{Rule Mining Algorithm}
    \label{alg:rule_mining}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\text
    bf{Output:}}
    \begin{algorithmic}[1]
        \REQUIRE Prediction $f = ⟨h,r,t⟩$, 
                 Facts from Training Set $\mathcal{G}$
        \ENSURE Candidate Rule Set for Prediction $\Phi$

        \STATE $\Phi \leftarrow \emptyset$
        \STATE \COMMENT{Step 1: CP Rule Extraction}
        \STATE $P \leftarrow \text{BFSSearch}(h, t)$
        \STATE $P_{rel} \leftarrow \text{CondensePath}(P)$
        \FOR{each $p$ in $P_{rel}$}
            \STATE $h, h', t, t' \leftarrow \text{localOptimization}(f, p, \mathcal{G})$
            \STATE $Rel_h\leftarrow 1 - \frac{f_r(h', t)}{f_r(h, t)},\quad Rel_t\leftarrow 1 - \frac{f_r(h, t')}{f_r(h, t)}$
            \IF{$Rel_h > 0$ \textbf{and} $Rel_t > 0$}
                \STATE $(HC, SC, supp) \leftarrow \text{RuleMetrics}(r\leftarrow p, \mathcal{G})$
                \IF{$SC \geq minSC$ \textbf{and} $HC \geq minHC$}
                    \STATE $\Phi \leftarrow \Phi \cup \{\phi_{CP}: r \leftarrow p [SC \times \frac{supp}{supp+minSupp}] \}$
                \ENDIF
            \ENDIF
        \ENDFOR

        \STATE \COMMENT{Step 2: PT Rule Extraction (Take Head PT Rule as Example)}
        \STATE $headTriples \leftarrow \text{SearchRelations}(h, \mathcal{G})$
        \FOR{each $⟨h,r',t'⟩$ in $headTriples$}
            \STATE $(HC, SC, supp) \leftarrow \text{RuleMetrics}(r(X, t)\leftarrow r'(X, t'), \mathcal{G})$
            \IF{$SC \geq minSC$ \textbf{and} $HC \geq minHC$}
                \STATE $\Phi \leftarrow \Phi \cup \{\phi_{PT}: r(X, t) \leftarrow r'(X, t') [SC \times \frac{supp}{supp+minSupp}] \}$
            \ENDIF
        \ENDFOR

        \RETURN $\Phi$
    \end{algorithmic}
\end{algorithm}


To generate path-based explanations, the eXpath method first extracts two types of rules—CP and PT rules, as defined in Section 4.1. Unlike KGEAttack, which mines all possible rules across the entire KG, eXpath focuses on rules specifically related to the given prediction. Rules relevant to a prediction necessarily arise from the relation paths between the head and tail entities of the predicted triple. As illustrated in Fig.~\ref{rulemining} and detailed in Algorithm~\ref{alg:rule_mining}, eXpath first searches for paths between the head and tail entities in the knowledge graph, filters these paths using a local optimization method to identify candidate rules, and finally evaluates their significance through a matrix-based approach.

In the first step, eXpath employs breadth-first search (BFS) to identify paths connecting the head and tail entities. To maintain interpretability, the maximum path length is limited to 3. Longer paths are not only harder to interpret but, as shown in prior research~\cite{meilicke2021naive}, are also less effectively represented by KGE models, making them unsuitable for explaining model predictions. Once identified, the paths are compressed into "relation paths" by omitting intermediate entities. This abstraction significantly reduces the number of candidates while retaining the essential semantic structure of the paths.

In the second step, eXpath filters the relation paths to determine their suitability as candidate rules. The filtering process is based on the importance of the head relation (the first hop in the relation path) and the tail relation (the last hop). Each relation path is assigned a head relevance and tail relevance score, reflecting its importance to the prediction. Relation paths where both the head and tail relevance scores are greater than zero are considered significant and are retained as the body of candidate rules for further evaluation. This rule-filtering approach is grounded in the assumption that a relation path can only serve as a valid rule body if both its head and tail relations are critical to the prediction.

To compute relevance scores, eXpath removes all facts associated with a specific relation and retrains the embedding model, observing the resulting drop in predictive performance. A substantial decline indicates that the relation is critical, and the extent of the decline quantifies its importance. However, retraining the entire model for each relation is computationally prohibitive. To address this, eXpath adopts a more efficient local optimization approach inspired by the Kelpie mimic strategy~\cite{rossi2022explaining}. Mimic entities for the head and tail, denoted as $h'$ and $t'$ (see Fig.~\ref{rulemining}(b)), are created. These mimic entities retain the same connections as the original head or tail entities, except that all facts associated with the relation being evaluated are removed. The embeddings of the mimic entities, along with those of the original head and tail entities, are then independently trained using their directly connected facts. 

Three predictive scores are calculated: $f_r(h, t)$, $f_r(h', t)$, and $f_r(h, t')$, where $f_r(h, t)$ is the model’s scoring function for the triple $⟨h, r, t⟩$. The relevance of a relation is computed using the following formulas:

\begin{equation}
\label{eq:relevance}
    Rel_h = 1 - \frac{f_r(h', t)}{f_r(h, t)}, \quad Rel_t = 1 - \frac{f_r(h, t')}{f_r(h, t)}.
\end{equation}

Here, $Rel_h$ and $Rel_t$ quantify the importance of relations linked to the head and tail entities, respectively. To ensure consistency across models and datasets, relative changes in scores are used instead of rank reductions, as scores provide a more robust metric. Rank reductions can be unreliable, especially in local optimization scenarios where mimic entities may overfit, producing consistent ranks of 1. Score reductions, however, align closely with accuracy declines observed under global optimization.

In the third step, eXpath constructs a candidate rule set $\Phi(f)$ for each prediction $f$, based on the filtered relation paths. The framework evaluates and selects high-quality rules with strong support and confidence. Confidence is computed as the product of standard confidence (SC) and a support coefficient. This approach prevents overestimation of rules with minimal support (e.g., supp $< 10$), which could otherwise disproportionately inflate their weight and lead to unreasonable fact selection. Strong support and confidence ensure the robustness of the selected rules for causal reasoning, enabling eXpath to generate accurate and interpretable path-based explanations.

Calculating metrics for PT rules is relatively straightforward and will not be elaborated here. However, efficiently computing the metrics for CP rules presents a key challenge. For this, we adopt the matrix-based approach from RLvLR~\cite{omran2019embedding}, which enables efficient evaluation of SC and HC for CP rules. 

To compute the metrics for CP rules, the method verifies the satisfiability of the body atoms in candidate rules. Given a KG represented as a set of \( S \) matrices, where each \( n \times n \) binary matrix \( S(r_k) \) corresponds to a relation \( r_k \), the adjacency matrix \( S(r_k) \) has an entry of 1 if the fact \( \langle e_i, r_k, e_j \rangle \) exists in the KG, and 0 otherwise. 

The product of adjacency matrices is closely related to closed-path rules. For instance, consider the rule \( \phi: r_t \leftarrow r_1, r_2 \). A fact \( r_t(e, e') \) is inferred by \( \phi \) if there exists \( e'' \) such that \( r_1(e, e'') \) and \( r_2(e'', e') \) hold. The product \( S(r_1) \cdot S(r_2) \) produces the adjacency matrix for the set of inferred facts. The binary transformation \( S(r_1, r_2) = \text{binary}(S(r_1) \cdot S(r_2)) \) is used to generalize this computation.

The metrics for CP rules are calculated as follows:

$$
\begin{aligned}
\text{supp}(\phi) = \text{sum}(S(r_1, r_2) \& S(r_t)) \\
\text{SC}(\phi) = \frac{\text{supp}(\phi)}{\text{sum}(S(r_1, r_2))},\text{HC}(\phi) &= \frac{\text{supp}(\phi)}{\text{sum}(S(r_t))}
\end{aligned}
$$

Here, \( \text{sum} \) aggregates all matrix entries, and \( \& \) represents element-wise logical AND. While this example involves rules of length 2, the method extends straightforwardly to rules of any length. This matrix-based approach provides a scalable solution for efficiently computing rule metrics in large knowledge graphs.

\subsection{Fact Selection} 

This section details the method for selecting an optimal set of facts to explain a given prediction triple \( \langle h, r, t \rangle \), leveraging the rules extracted in the previous step. The core idea is to identify the most critical fact or a combination of facts within the paths connecting the head and tail entities. Each fact is evaluated based on its contribution to the prediction, and those with higher scores are considered more pivotal. The final explanation set is constructed by selecting the highest-scoring facts.

To determine the significance of a fact, several key factors are taken into account. The scoring method incorporates the following preferences:
\begin{itemize}
    \item Facts that satisfy a larger number of rules are given higher priority, as this indicates their broader relevance within the prediction.
    \item Rules with higher confidence are weighted more heavily, reflecting their stronger causal support.
    \item The position of a fact within a rule (e.g., whether it connects to the head or tail entity) is adjusted based on the relation relevance scores determined earlier. This ensures that facts aligned with the critical relations are appropriately emphasized.
\end{itemize}

By combining these factors, the scoring system provides a robust metric for evaluating each fact's importance. To model the contribution of a fact that satisfies multiple rules, we adopt a confidence degree (CD) aggregation approach inspired by rule-based link prediction methods~\cite{omran2018scalable}. The CD of a fact \( f \) is calculated using the SC (standard confidence) values of all the rules that infer \( f \) in a Noisy-OR manner. For explanation tasks, which reverse the link prediction perspective, we define the CD of \( f \) as follows:

\[
C D(f) = 1 - \prod_{\phi \in \Phi}(1 - c(\phi) \cdot w(f, \phi)),
\]

where \( \Phi \) is the set of rules inferred from the prediction, \( c(\phi) \) is the confidence of rule \( \phi \), and \( w(f, \phi) \) represents the importance of fact \( f \) within rule \( \phi \). This importance score, ranging from 0 to 1, reflects both the proportion of \( f \)'s appearances in the rule and its relative importance based on the relevance of the rule's head and tail relations. 

The importance score \( w(f, \phi) \) is calculated as:

$$
\begin{aligned}
r_h(\phi) &= \frac{Rel_h(\phi)}{Rel_h(\phi) + Rel_t(\phi)}\\
w(f, \phi) &= r_h(\phi) \cdot p_h(f, \phi) + (1 - r_h(\phi)) \cdot p_t(f, \phi)
\end{aligned}
$$

where \( Rel_h(\phi) \) and \( Rel_t(\phi) \) are the relevance scores of the rule's head and tail relations, respectively. The term \( p_h(f, \phi) \) represents the proportion of \( f \)'s appearances in the rule's head relation. This formulation ensures that facts appearing more prominently in rules with important head relations are scored higher.

This method applies to CP, and PT rules, though it simplifies for PT. For example, in head PT rules, \( r_h(\phi) = 1 \) and \( p_h(f, \phi) = 1 \), so \( w(f, \phi) = 1 \).

We rank all candidate facts by their CD scores and select the top-ranked facts to form the explanation. This approach ensures that the selected facts are those most strongly supported by high-quality, relevant rules, providing robust and interpretable explanations for the given prediction.




==> backup/tex/5_experiment.tex <==
\section{Experiment}
\subsection{Experimental Setup}

We assessed eXpath on the KG LP task using four benchmark datasets: FB15k, FB15k-237 ~\cite{lacroix2018canonical}, WN18, and WN18RR ~\cite{bhowmik2020explainable}. These datasets' detailed statistics and link prediction metrics are provided in the table~\ref{tab:dataset}. We adhered to the standard splits and training parameters to ensure consistency across comparisons, except in cases where training time posed a challenge. Specifically, we reduced the number of epochs for four settings to avoid an impractically long experimental duration (which would have required several months). This underfitting led to some degradation in LP metrics for these settings but does not affect the fairness of the explanations since the adversarial LP explanation experiments maintain identical training parameters before and after removing facts.


\begin{table}[htbp]
\centering
\caption{Statistics of benchmark datasets.}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrr}
\toprule
\makecell[c]{KG\\Dataset} & 
\makecell[c]{Entities} & 
\makecell[c]{Relation\\Types} & 
\makecell[c]{Train\\Facts} & 
\makecell[c]{Valid\\Facts} & 
\makecell[c]{Test\\Facts} \\
\midrule
FB15k       & 14,951   & 1,345          & 483,142     & 50,000      & 50,971     \\
FB15k-237   & 14,541   & 237            & 272,115     & 17,535      & 20,466     \\
WN18        & 40,943   & 18             & 141,442     & 5,000       & 5,000      \\
WN18RR      & 40,943   & 11             & 86,835      & 3,034       & 3,134      \\
\bottomrule
\end{tabular}
\label{tab:dataset}
\end{table}


We compared the performance of eXpath against four contemporary systems dedicated to LP interpretation: Kelpie~\cite{rossi2022explaining}, Data Poisoning (DP)~\cite{zhang2019data}, Criage~\cite{betz2022adversarial}, and KGEAttack~\cite{betz2022adversarial}. These implementations are publicly available, and we tailored the code sourced from their respective Github repositories. Since the explanation framework is compatible with any Link Prediction (LP) model rooted in embeddings, we conduct experiments on two models with different loss functions: CompEx~\cite{trouillon2016complex}, ConvE~\cite{dettmers2018convolutional}, and TransE~\cite{wang2014knowledge}.

The task for this experiment is path-based adversarial LP explanation: each explanation framework recommends one or more facts, and these facts are removed before retraining the model with the same parameters. The drop in performance metrics is used to assess the quality of the explanations. The baseline frameworks, including DP, Criage, Kelpie(L1), and Kelpie, focus solely on facts directly related to the head entity (i.e., attributes of the head entity), KGEAttack randomly selects a fact in the extracted rule, whereas eXpath focuses on facts related to either the head or tail entity, each supported by relevant CP, Uc rules. To ensure fairness between the explanation systems, we restrict the number of facts that can be removed. Specifically, DP, Criage, Kelpie(L1), and eXpath(L1) limit the removal to at most one fact, whereas Kelpie and eXpath can remove up to four facts. Based on experiments and existing literature, we set the thresholds \( \text{minSC} = 0.01, \text{minHC} = 0.01, \text{minSupp} = 10 \). These parameters are adapted from the definitions of high-quality rules in prior work (e.g., \( \text{SC} \geq 0.1 \) and \( \text{HC} \geq 0.01 \) in [Galárraga et al., 2015]) and further tuned for our framework.

Based on the problem formulation defined in Section 3.3, we randomly select a small subset \( T \subset \mathcal{G}_e \) from the test set, where the model demonstrates relatively good predictive performance. Specifically, we randomly select 100 predictions that exhibit relatively strong performance. Note that these predictions are not required to rank first for both head and tail predictions, as such strict conditions could overly constrain the selection process, thereby limiting the applicability of the scenarios. According to the definition of \( \delta MRR(M_x, T) \), predictions with lower performance have a smaller weight in the evaluation.

The model's explanatory capability is measured by the degradation in H@1 (Hits@1) and MRR (Mean Reciprocal Rank), expressed as:

\begin{equation}
\label{eq:delta_mrr}
\begin{aligned}
H@1(M_x,f) &=\frac{1}{2}(\mathbf{1}(rk_h(M_x,f)=1) + \mathbf{1}(rk_t(M_x,f)=1)) \\
RR(M_x, f) &= \frac{1}{2} \left( \frac{1}{rk_h(M_x, f)} + \frac{1}{rk_t(M_x, f)} \right) \\
\delta H@1(M_x, T) &= 1 - \frac{\sum_{f\in T} H@1(M_x,f)}{\sum_{f\in T} H@1(M_o,f)} \\
\delta MRR(M_x, T) &= 1 - \frac{\sum_{f\in T} RR(M_x,f)}{\sum_{f\in T} RR(M_o,f)}
\end{aligned}
\end{equation}

Where \( M_x \) represents the model trained on the dataset excluding the candidate explanations extracted by the explanation framework \( x \), and \( M_o \) denotes the original model trained on the entire dataset, $\mathbf{1}(\cdot)$  is the indicator function that returns 1 if the condition inside holds true and 0 otherwise. We adopt the relative reduction in reciprocal rank instead of the absolute reduction since the predictions in \( T \) are not necessarily top-ranked for both head and tail predictions. 

To ensure that the prediction to be explained is of high quality, we restrict the MRR to \( > 0.5 \), which ensures that the prediction ranks first in at least one of the head or tail predictions. As Equation ~\ref{eq:delta_mrr}, to evaluate the overall explanatory power, we sum the MRR values of new model \( M_x \) and original model \( M_o \) across all facts in the numerator and denominator, respectively. This approach ensures that better predictions contribute more significantly to the evaluation, avoiding a bias toward only selecting predictions where both head and tail ranks are 1. Moreover, this method allows for negative explanations, where the rank decreases after removing a fact.


To further compare the performance of two explanation frameworks, we calculate the proportion of predictions where \( M_x \) provides better explanations than \( M_y \), and by how much. These metrics provide insights into the relative explanatory capabilities of the two frameworks, both in terms of the proportion of predictions where one framework outperforms the other and the magnitude of the improvement.

\subsection{Explanation Results}

\begin{table*}[h!]
\centering
\caption{$\delta H@1$ comparison across different models and datasets using various explanation methods. All results are averaged over five runs, with higher values indicating better performance. The original $H@1$ is 1 for all candidate predictions ($H@1 > 1$ predictions are excluded from the metric). Methods with "+X" indicate fusion approaches that combine the given method with eXpath.}
\label{tab:deltaH1}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{\makecell[c]{Max \\ Exp. \\ Size}} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Complex} & \multicolumn{4}{c}{Conve} & \multicolumn{4}{c}{TransE} & \multirow{2}{*}{AVG} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} & \\
\midrule
\multirow{9}{*}{\makecell[c]{single\\-fact\\methods}} & Criage & .087 & .105 & .080 & .203 & .153 & .162 & .270 & .256 & --- & --- & --- & --- & .165 \\
 & DP & .529 & .315 & .799 & .758 & .246 & .162 & .794 & .829 & .304 & .326 & .910 & .709 & .557 \\
 & Kelpie & .576 & .395 & .578 & .593 & .229 & .222 & .567 & .667 & .261 & .281 & .792 & .779 & .495 \\
 & AnyBurl & .547 & .290 & .829 & .764 & .237 & .212 & \underline{.929} & \underline{.915} & .365 & .213 & .938 & .779 & .585 \\
 & eXpath & .512 & .395 & .834 & .797 & .271 & .343 & \underline{.929} & .891 & .313 & .337 & .938 & .767 & .611 \\
 & Criage+eXPath & .523 & .411 & .839 & \underline{.819} & .322 & .404 & \textbf{.936} & .891 & --- & --- & --- & --- & .643 (+290\%)  \\
 & DP+eXpath & .570 & \underline{.500} & \textbf{.859} & .813 & \underline{.331} & \underline{.414} & \textbf{.936} & \textbf{.946} & .374 & \textbf{.438} & \textbf{.944} & .826 & \underline{.663} (+19\%) \\
 & Kelpie+eXPath & \textbf{.657} & \textbf{.540} & \textbf{.859} & \textbf{.835} & \textbf{.364} & \textbf{.424} & .929 & \underline{.915} & \textbf{.417} & \underline{.427} & \textbf{.944} & \textbf{.872} & \textbf{.682} (+38\%) \\
 & AnyBurl+eXpath & \underline{.576} & .452 & \textbf{.859} & .802 & .322 & .384 & .929 & \textbf{.946} & \textbf{.417} & .360 & .938 & \textbf{.872} & .655 (+12\%) \\
\midrule
\multirow{3}{*}{\makecell[c]{four\\-fact\\methods}} & Kelpie & .767 & .581 & .829 & .940 & .534 & .303 & .816 & .946 & .374 & .427 & .868 & .907 & .691 \\
 & eXpath & \underline{.802} & \underline{.661} & \underline{.920} & \underline{.951} & \underline{.542} & \underline{.566} & \underline{.957} & \underline{.984} & \underline{.539} & \underline{.573} & \textbf{.965} & \textbf{.965} & \underline{.785} \\
 & Kelpie+eXpath & \textbf{.831} & \textbf{.742} & \textbf{.935} & \textbf{.989} & \textbf{.653} & \textbf{.596} & \textbf{.965} & \textbf{.984} & \textbf{.609} & \textbf{.674} & \textbf{.965} & \textbf{.965} & \textbf{.826} \\
\bottomrule
\end{tabular}
\end{table*}



\begin{table*}[h!]
\centering
\caption{$\delta MRR$ comparison across different models and datasets using various explanation methods. All results are averaged over five runs, with higher values indicating better performance. The original MRR is above 0.5 in all candidate predictions.}
\label{tab:deltaMRR}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{\makecell[c]{Max \\ Exp. \\ Size}} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Complex} & \multicolumn{4}{c}{Conve} & \multicolumn{4}{c}{TransE} & \multirow{2}{*}{AVG} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} & \\
\midrule
\multirow{9}{*}{\makecell[c]{single\\-fact\\methods}} & Criage & .045 & .051 & .058 & .163 & .024 & .031 & .157 & .150 & --- & --- & --- & --- & .085 \\
 & DP & .451 & .187 & .729 & .668 & .140 & .058 & .728 & .785 & .157 & .141 & .742 & .613 & .450 \\
 & Kelpie & .457 & .238 & .491 & .483 & .123 & .076 & .514 & .578 & .075 & .115 & .700 & .664 & .376 \\
 & AnyBurl & .463 & .172 & .766 & .684 & .159 & .104 & .889 & .853 & .190 & .091 & .877 & .659 & .492 \\
 & eXpath & .430 & .233 & .774 & .688 & .183 & .130 & .889 & .810 & .159 & .165 & .877 & .596 & .494 \\
 & Criage+eXpath & .443 & .236 & .777 & .711 & .203 & .185 & .892 & .814 & --- & --- & --- & --- & .533 (+527\%) \\
 & DP+eXpath & .491 & \underline{.282} & \textbf{.803} & .711 & \underline{.241} & \underline{.211} & \textbf{.900} & \textbf{.893} & \underline{.239} & \textbf{.252} & \underline{.891} & .675 & \underline{.549} (+22\%) \\
 & Kelpie+eXpath & \textbf{.534} & \textbf{.309} & .795 & \textbf{.718} & \textbf{.245} & .206 & \underline{.895} & .848 & .225 & \underline{.239} & \textbf{.893} & \textbf{.734} & \textbf{.553} (+47\%) \\
 & AnyBurl+eXpath & \underline{.495} & .262 & \underline{.799} & \underline{.712} & .239 & \textbf{.215} & .889 & \underline{.883} & \textbf{.261} & .223 & .877 & \underline{.723} & .548 (+12\%) \\
\midrule
\multirow{3}{*}{\makecell[c]{four\\-fact\\methods}} & Kelpie & .632 & .434 & .777 & \underline{.891} & \underline{.391} & .143 & .795 & .919 & .203 & .199 & .805 & .893 & .590 \\
 & eXpath & \underline{.680} & \underline{.452} & \underline{.875} & .887 & .366 & \underline{.327} & \underline{.924} & \underline{.952} & \underline{.354} & \underline{.261} & \underline{.937} & \underline{.943} & \underline{.663} \\
 & Kelpie+eXpath & \textbf{.718} & \textbf{.519} & \textbf{.900} & \textbf{.941} & \textbf{.468} & \textbf{.401} & \textbf{.949} & \textbf{.966} & \textbf{.406} & \textbf{.332} & \textbf{.952} & \textbf{.960} & \textbf{.709} \\
\bottomrule
\end{tabular}
\end{table*}


Tables ~\ref{tab:deltaH1} and ~\ref{tab:deltaMRR} demonstrate the effectiveness of the eXpath method in generating explanations for link prediction tasks, evaluated using the $\delta H@1$ and $\delta MRR$ metrics as defined in Equation~\ref{eq:delta_mrr}. The best and second-best results are highlighted in \textbf{bold} and \underline{underlined}, respectively.

To ensure fair comparison, explanation methods are grouped by explanation size (i.e., the number of facts provided). The first section of each table (top 9 rows) presents results for five single-fact methods (L1 methods) and their fusion models, such as Criage, DP, Kelpie, KGEAttack, and eXpath, which offer one fact per explanation. The second section (bottom 3 rows) shows results for four-fact methods (L4 methods), including eXpath(L4), Kelpie(L4), and their fusion. While Kelpie supports explanations of lengths 1 and 4, eXpath is flexible and can generate explanations of any length based on the specified configuration.

As shown in Tables ~\ref{tab:deltaH1} and ~\ref{tab:deltaMRR}, eXpath(L1) consistently outperforms state-of-the-art models across datasets and LP models. Among single-fact methods, eXpath(L1) delivers the best average performance, achieving a 0.67 reduction in $\delta H@1$ and a 0.49 reduction in $\delta MRR$. KGEAttack performs comparably, followed by DP and Kelpie(L1), while Criage performs the worst. eXpath(L1) secures at least the second-best performance in 20 out of 24 settings and significantly outperforms all methods in 12 settings. For example, on ConvE with FB15k-237, eXpath(L1) surpasses Kelpie(L1) by 25\% in $\delta MRR$ and 62\% in $\delta H@1$. Similarly, on ConvE with FB15k, eXpath(L1) exceeds KGEAttack by 15\% in $\delta MRR$ and 14\% in $\delta H@1$.

Interestingly, different explanation methods exhibit dataset-specific preferences. For instance, eXpath(L1) performs well on WN18 and FB15k-237 but struggles on WN18RR. Conversely, KGEAttack excels on WN18 and WN18RR but performs poorly on FB15k-237. These results suggest that attack efficacy and KGE robustness depend heavily on dataset characteristics. Dense graphs like FB15k and FB15k-237 retain redundant evidence even after triple removal, reducing the attack’s impact. Conversely, sparser datasets like WN18RR favor simpler attack strategies.

Kelpie(L4), which considers interactions among facts, consistently outperforms single-fact methods in almost all settings, underscoring the importance of multi-fact combinations for satisfactory explanations. However, eXpath(L4), which directly selects the top-scoring set of up to four facts, surpasses Kelpie(L4) in 10 out of 12 settings with statistical significance ($p$-value $<0.05$) over five runs. While Kelpie relies on combinatorial searches, eXpath’s scoring-based fact selection achieves superior performance without interaction effects. For dense datasets like FB15k and FB15k-237, multi-fact explanations yield over a 70\% improvement compared to single-fact explanations. However, in sparser datasets like WN18 and WN18RR, single-fact explanations offer only a 20\% improvement.

Dense graphs like FB15k include numerous redundant and near-inverse relations (e.g., \texttt{actor-film}, \texttt{sequel-prequel}, \texttt{award-honor}). Removing one fact often leaves other facts that still support the prediction, as shown in Figure~\ref{example}. This observation highlights the need for multi-fact explanations to address the predictive context fully.

We also introduce theoretical fusion methods (e.g., Kelpie+eXpath), which combine the best explanations from two methods for each prediction by selecting the explanation that yields the greater reduction in MRR, defined as $RR(M_{x+y}, f) = \min(RR(M_x, f), RR(M_y, f))$. Such methods emphasize the complementary strengths of different approaches and demonstrate the potential for a theoretically superior method.

Fusion methods significantly enhance explanation performance. For instance, combining eXpath(L1) with Criage, DP, Kelpie(L1), and KGEAttack improves $\delta MRR$ by 527\%, 22\%, 47\%, and 12\%, respectively. The eXpath-Kelpie fusion improves Kelpie alone by 20\%. These results demonstrate that eXpath offers diverse and complementary perspectives, particularly when integrated with Kelpie, highlighting differences in explanation strategies. However, L1 fusion methods converge to an upper bound ($\delta MRR=0.55, \delta H@1=0.68$), indicating that single-fact explanations have inherent limitations. Multi-fact approaches are necessary for satisfactory explanations in link prediction tasks.

While both $\delta H@1$ and $\delta MRR$ are useful, $\delta MRR$ proves more robust. The stochasticity of model training and small dataset size (100 predictions) can cause significant variability in $\delta H@1$ values. For instance, rank differences between 1 and 2 directly impact $\delta H@1$ by 0.01, leading to higher variance. This issue is exacerbated for fragile models like TransE, where ranks fluctuate even without attacks. We address this by averaging results over five experimental runs and repeating subsets of experiments on five distinct samples of 100 tail predictions each. Results from these repetitions closely align with the values reported here, as detailed in our online repository.


\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{pic/superiorV3.png}
\caption{Percentage of predictions that eXpath provide superior explanations.} \label{superior}
\end{figure*}

The diversity of eXpath's explanations is further evidenced in Figure~\ref{fig:explanation_diversity}, which illustrates the proportion of predictions where eXpath provides better explanations than other systems (i.e., greater rank reduction, $RR(M_x, f) < RR(M_y, f)$) among all valid explanations. Across all datasets and models, eXpath(L1) achieves better explanations in an average of 34.6\%, 44.2\%, and 28.4\% of predictions compared to DP, KGEAttack, and Kelpie(L1), respectively. For eXpath(L4), the proportion increases to an average of 37.6\%. Notably, eXpath demonstrates the highest relative improvement on the FB15k-237 dataset, where it provides better explanations for 48.8\% of predictions.

In comparison to Table~\ref{tab:deltaMRR}, these results reveal an interesting phenomenon: even though eXpath does not always achieve the highest overall $\delta MRR$, it performs significantly better on many individual predictions. This indicates that explanation tasks, unlike prediction tasks, do not have a single definitive outcome. Multiple explanations may lead to successful attacks, and the effectiveness of a method depends on its preferences and scope. For instance, eXpath is well-suited for path-based explanations, Kelpie excels in fact-based explanations, and KGEAttack is effective for rule-based explanations. While these methods share some conceptual overlap, their generated explanations exhibit substantial diversity, as further illustrated in Section~\ref{sec:case_study}. This diversity underscores the complementary strengths of different explanation approaches and highlights the importance of selecting the appropriate method for the specific characteristics of the link prediction task and dataset.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{pic/timeV1.png}
\caption{Average times in seconds to extract a explanation for Kelpie and eXpath.} \label{time}
\end{figure}

In terms of efficiency, Figure~\ref{time} compares the average explanation time per prediction between eXpath and Kelpie. eXpath achieves significantly faster explanation speeds, averaging 25.61 seconds per prediction, which is less than 40\% of Kelpie's average time of 66.36 seconds. This efficiency is attributed to eXpath's localized optimization within relation groups and its straightforward scoring-based fact selection process, compared to Kelpie's exhaustive traversal of connections and time-intensive combinatorial searches.

In conclusion, eXpath demonstrates clear advantages in both performance and execution efficiency, establishing a new benchmark for accuracy and speed in explanation generation. These results highlight its potential as a robust framework for advancing path-based and rule-based explanation systems in link prediction tasks.

\subsection{Fact Position Preferences}

\begin{table*}[h!]
\centering
\caption{$\delta MRR$ Comparison between different models and datasets. All results are averages over five runs. Greater is better. The original MRR is above 0.5 in all candidate predictions.}
\label{tab:preference}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{\makecell[c]{Max \\ Exp. \\ Size}} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Complex} & \multicolumn{4}{c}{Conve} & \multicolumn{4}{c}{TransE} & \multirow{2}{*}{AVG} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} & \\
\midrule
\multirow{3}{*}{1} 
 & eXpath(all) & .431 & .233 & \textbf{.774} & .696 & .163 & \textbf{.135} & \textbf{.889} & \textbf{.833} & \textbf{.159} & \textbf{.149} & \textbf{.877} & .406 & .479 \\
 & eXpath(head) & .433 & \textbf{.243} & \textbf{.774} & .693 & .165 & .119 & \textbf{.889} & .810 & .148 & .127 & \textbf{.877} & \textbf{.598} & \textbf{.490} \\
 & eXpath(tail) & \textbf{.448} & .125 & .759 & \textbf{.635} & \textbf{.177} & .088 & \textbf{.889} & .787 & .159 & .071 & \textbf{.877} & -.059 & .413 \\
\midrule
\multirow{3}{*}{2} 
 & eXpath(all) & .520 & \textbf{.343} & .783 & \textbf{.809} & .230 & .196 & \textbf{.888} & .900 & .231 & .177 & .904 & .602 & .549 \\
 & eXpath(head) & \textbf{.539} & .329 & .780 & .769 & .223 & .196 & \textbf{.889} & \textbf{.902} & \textbf{.254} & \textbf{.251} & \textbf{.908} & \textbf{.820} & \textbf{.572} \\
 & eXpath(tail) & .549 & .156 & \textbf{.784} & .737 & \textbf{.291} & \textbf{.134} & .885 & .869 & .227 & .134 & .857 & .000 & .469 \\
\midrule
\multirow{3}{*}{4} 
 & eXpath(all) & \textbf{.680} & \textbf{.453} & .807 & .878 & .370 & \textbf{.319} & .900 & .939 & \textbf{.355} & .270 & .918 & .826 & .643 \\
 & eXpath(head) & .659 & .438 & \textbf{.877} & \textbf{.887} & \textbf{.372} & .290 & \textbf{.925} & \textbf{.952} & .346 & \textbf{.271} & \textbf{.935} & \textbf{.942} & \textbf{.658} \\
 & eXpath(tail) & .630 & .227 & .833 & .818 & .324 & .103 & .877 & .859 & .232 & .135 & .843 & .125 & .501 \\
\midrule
\multirow{3}{*}{8} 
 & eXpath(all) & \textbf{.762} & \textbf{.584} & .850 & .956 & .449 & .419 & .930 & .961 & .471 & .333 & .932 & .909 & .713 \\
 & eXpath(head) & .727 & .558 & .904 & \textbf{.990} & .438 & .394 & .919 & \textbf{.978} & \textbf{.533} & \textbf{.350} & \textbf{.965} & \textbf{.959} & \textbf{.726} \\
 & eXpath(tail) & .737 & .337 & \textbf{.927} & .920 & \textbf{.450} & \textbf{.240} & \textbf{.927} & .913 & .389 & .201 & .923 & .367 & .611 \\
\bottomrule
\end{tabular}
\end{table*}

To evaluate the effect of restricting facts to either the head or tail entity, we investigated whether such constraints impact link prediction performance. This analysis explores the relative significance of head and tail entity attributes, which often depend on dataset characteristics. Table~\ref{tab:preference} shows the impact of these restrictions across different explanation sizes (1, 2, 4, 8). Here, \texttt{all} denotes unrestricted fact selection, \texttt{head} restricts facts to those connected to the head entity, and \texttt{tail} restricts facts to those connected to the tail entity. Facts unrelated to either the head or tail entity are not considered as they do not directly influence their embeddings.

On average, restricting facts to head entities (\texttt{head}) yields better performance than unrestricted selection (\texttt{all}) across explanation sizes, while restricting to tail entities (\texttt{tail}) consistently results in weaker performance. Notably, \texttt{head} achieves the highest average performance for most settings, but the benefits are dataset- and model-specific. For example, in the case of explanation size 1, \texttt{all} slightly underperforms compared to \texttt{head} only in TransE with WN18RR (\texttt{head: 0.598} vs. \texttt{all: 0.406}), largely due to the dataset and model’s inherent bias. Interestingly, in this specific setting, \texttt{tail} performs exceptionally poorly (\texttt{tail: -0.059}), being the only configuration where MRR increases after the attack, indicating ineffective explanations.

Dataset characteristics play a significant role in determining the effectiveness of fact restrictions. For FB15k and FB15k-237, \texttt{all} generally performs slightly better than \texttt{head}, but the differences are not pronounced. In certain cases, such as with the TransE model, \texttt{head} outperforms \texttt{all}. In contrast, for WN18 and WN18RR, restricting to head-related facts (\texttt{head}) significantly improves performance. This is likely because FB15k and FB15k-237 are dense graphs with high fact/entity ratios, encouraging models to balance head and tail entity modeling and reducing reliance on a single direction. In sparser datasets like WN18 and WN18RR, the head entity tends to hold greater significance, as it often represents central concepts, while tail entities often act as hubs with numerous connections.

Restricting to tail-related facts (\texttt{tail}) results in consistently weaker performance across all datasets, with significant average drops observed in FB15k-237 (-50\%) and WN18RR (-40\%) compared to \texttt{head}. Exceptions are limited to explanation size 1 on FB15k, where \texttt{tail} performs slightly better. For FB15k and WN18, which do not remove inverse relations, the differences between \texttt{head} and \texttt{tail} are less pronounced, with \texttt{tail} showing only a 9\% decline compared to \texttt{head}. This variation highlights the roles of head and tail entities in different datasets: head entities often represent general or central concepts (e.g., "person" or "organization"), while tail entities frequently act as hubs (e.g., "male," "New York," or "CEO") with numerous connections. Removing facts associated with hub entities has limited impact on prediction metrics due to their less central contextual roles.

Different models exhibit varying sensitivities to fact restrictions. Restricting to tail-related facts leads to average performance drops of 8.2\%, 15\%, and 41\% for ComplEx, ConvE, and TransE, respectively, compared to \texttt{head}. TransE, with its translational operation, strongly relies on head entity and relation embeddings, making it particularly sensitive to head-related contexts and highly biased. ConvE shares similar biases but to a lesser extent, while ComplEx models symmetrical interactions between head, relation, and tail, achieving more balanced performance. However, even ComplEx shows an 8.2\% drop, suggesting that dataset characteristics, rather than model design alone, play a significant role in determining fact preferences.

Fact restrictions should align with dataset-specific characteristics to ensure focused and meaningful explanations. Tailoring restrictions based on graph density offers a practical heuristic. Using the fact/entity ratio as a measure of density, we applied head fact restrictions for low-density datasets (ratio $<$ 10, i.e., WN18 and WN18RR) but used unrestricted selection for high-density datasets (ratio $>$ 10, i.e., FB15k and FB15k-237) to balance performance and explanation richness. While Kelpie inherently restricts explanations to head-related facts, such constraints may limit diversity and the semantic richness of explanations. Our findings emphasize the importance of flexibility in explanation strategies, enabling them to adapt to the unique properties of datasets and models.


\subsection{Ablation Study}

\begin{table*}[h!]
\centering
\caption{Ablation study results on $\delta \text{MRR}$, comparing the impact of excluding CP rules (\textbf{w/o CP}) and Uc rules (\textbf{w/o Uc}) across different models and datasets. The \textbf{Sparse} strategy selects facts associated with the sparsest relations as explanations, serving as a baseline for comparison. }
\label{tab:ablation}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{\makecell[c]{Max \\ Exp. \\ Size}} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Complex} & \multicolumn{4}{c}{Conve} & \multicolumn{4}{c}{TransE} & \multirow{2}{*}{AVG} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} 
 & \rotatebox{60}{FB15k} & \rotatebox{60}{FB15k-237} & \rotatebox{60}{WN18} & \rotatebox{60}{WN18RR} & \\
\midrule
\multirow{4}{*}{1} & eXpath & .431 & .223 & .774 & .693 & .163 & .135 & .889 & .810 & .159 & .149 & .877 & .598 & .492 \\
 & eXpath (w/o CP) & \textbf{.276} & .195 & \textbf{.757} & \textbf{.659} & \textbf{.083} & \textbf{.125} & \textbf{.448} & \textbf{.423} & \textbf{.106} & \textbf{.153} & \textbf{.520} & \textbf{.574} & \textbf{.360} (-27\%) \\
 & eXpath (w/o Uc) & .431 & \textbf{.118} & .774 & .685 & .154 & .047 & .889 & .853 & .155 & .097 & .877 & .558 & .470 (-4.5\%) \\
\midrule
\multirow{4}{*}{4} & eXpath & .680 & .453 & .877 & .887 & .370 & .319 & .925 & .952 & .355 & .270 & .935 & .942 & .664 \\
 & eXpath (w/o CP) & \textbf{.477} & .416 & \textbf{.875} & .877 & \textbf{.212} & .295 & \textbf{.708} & \textbf{.835} & \textbf{.190} & \textbf{.276} & \textbf{.800} & \textbf{.936} & \textbf{.575} (-13.5\%) \\
 & eXpath (w/o Uc) & .622 & \textbf{.305} & .833 & \textbf{.839} & .341 & \textbf{.159} & .925 & .953 & .329 & .174 & .941 & .930 & .613 (-6\%) \\
\bottomrule
\end{tabular}
\end{table*}


To evaluate the effectiveness of the components of our approach, ablation experiments were conducted by removing one type of rule at a time for fact scoring, analyzing the individual contributions of the two scoring rules—CP and Uc—used in our method. Table~\ref{tab:ablation} presents the results for explanation sizes of 1 and 4. In the table, \texttt{eXpath} represents the full method using both CP and Uc rules, \texttt{eXpath(w/o CP)} indicates the method without CP rules, \texttt{eXpath(w/o Uc)} excludes Uc rules, and \texttt{eXpath(sparse)} applies a simple strategy that selects random facts associated with the sparsest relation (i.e., the relation with the fewest associated facts). 

The results show that removing either type of rule leads to performance drops, with reductions of 27\% and 13.5\% for CP rules and 4.5\% and 6\% for Uc rules, respectively. These findings underscore the critical role of CP rules in link prediction, serving as the primary mechanism for addressing complex relational patterns. Uc rules, while less impactful, significantly complement CP rules by improving the diversity and reliability of the explanations. Removing both CP and Uc rules and relying solely on relation sparsity (\texttt{eXpath(sparse)}) leads to the most substantial performance degradation with reductions of 30.5\% and 23.5\%, demonstrating the necessity of incorporating structured rules for effective fact scoring and explanation generation.

The impact of rule removal varies across datasets. For FB15k, CP rules prove most essential, with an average performance drop of 38\%, while Uc rules have minimal impact, suggesting that CP rules alone are sufficient to support most predictions in this dataset. On the other hand, in FB15k-237, Uc rules have the greatest influence, with an average drop of 42\%, whereas CP rules contribute less significantly. This discrepancy suggests that the denser and more diverse relational structures in FB15k-237 benefit from Uc rules. For WN18, CP rules show a significant effect, with an average performance drop of 23\%, reflecting the importance of capturing linguistic biases through CP rules in this dataset. Interestingly, for WN18RR, neither CP nor Uc rules individually cause significant performance degradation, but removing both rules simultaneously leads to a substantial drop. This observation indicates that CP and Uc rules are complementary, often providing overlapping support, especially in simpler datasets like WN18RR.

These results provide several key insights into the role of CP and Uc rules. CP rules are foundational for addressing linguistic biases and supporting most link predictions. Even without Uc rules, as in \texttt{eXpath(w/o Uc)}, the method can still recommend effective explanations, emphasizing the centrality of CP rules. Meanwhile, Uc rules serve as valuable complements, particularly in datasets with complex relational structures like FB15k-237, where their absence significantly impacts performance. Relying solely on relation relevance, as in \texttt{eXpath(rel)}, leads to the largest performance drop, underscoring the necessity of rule-based reasoning to go beyond simple relevance measures. Furthermore, the complementary nature of CP and Uc rules ensures robust performance, particularly in datasets like WN18RR. These findings demonstrate that while CP rules form the backbone of effective explanations, Uc rules enhance the overall credibility and diversity of predictions, particularly in datasets with diverse or dense relational structures.



\subsection{Case Study}



\begin{table*}[htbp]
\centering
\begin{tabular}{p{2.5cm} | p{2.5cm} | p{5.5cm} | p{6cm}}
\toprule
              Prediction &                                     KGEAttack &                                            kelpie &                                          eXpath \\
\midrule
     $e_0$, award\_nominee, $e_1$ \newline(from \texttt{complex FB15k}) & [0.89]\newline $e_1$, award, $e_0$ & [L1: 0.25/L4: 0.38]\newline $e_0$, award\_nominee, Anna\_Paquin\newline $e_0$, award\_nominee, Shohreh\_Aghdashloo\newline $e_0$, award\_nominee, Julia\_Ormond\newline $e_0$, award\_nominee, Amanda\_Plummer & [L1: 0.89/L4: 0.95]\newline $e_1$, award, $e_0$\newline $e_0$, award\_nominee, Joan\_Allen\newline Tony\_Award.., award\_nominee, $e_1$\newline Academy\_Award.., award\_nominee, $e_1$ \\
     \midrule
    Porco\_Rosso, country, Japan \newline(from \texttt{conve FB15k}) &        [0.00]\newline Anime, films\_in\_this\_genre, Porco\_Rosso &       [L1: 0.62/L4: 0.74]\newline Hayao\_Miyazaki, film, Porco\_Rosso\newline Porco\_Rosso, language, Japanese\_Language & [L1: 0.73/L4: 0.84]\newline Porco\_Rosso, language, Japanese\_Language\newline Hayao\_Miyazaki, film, Porco\_Rosso\newline Fantasy, titles, Porco\_Rosso\newline Porco\_Rosso, written\_by, Hayao\_Miyazaki \\
    \midrule
    $e_2$, medal, Silver\_medal \newline(from \texttt{complex FB15k-237}) &      [0.00]\newline Venezuela, olympics, $e_2$ & [L1: 0.00/L4: 0.00]\newline $e_2$, participating\_countries, United\_Kingdom\newline United\_States\_of\_America, olympics,  $e_2$\newline France, olympics, $e_2$ & [L1: 0.25/L4: 0.62]\newline $e_2$, medal, Bronze\_medal\newline 1976\_Summer\_Olympics, medal, Silver\_medal\newline 1976\_Winter\_Olympics, medal, Silver\_medal\newline 2008\_Summer\_Olympics, medal, Silver\_medal \\
    \midrule
    $e_3$, actor, Jonathan\_Pryce \newline(from \texttt{complex FB15k}) & [0.00]\newline $e_3$, prequel, $e_4$ & [L1: 0.00/L4: 0.58]\newline $e_4$, sequel, $e_3$\newline Keith\_Richards, film, $e_3$\newline $e_3$, actor, Keith\_Richards\newline Action\_Film, films\_in\_this\_genre, $e_3$ & [L1: 0.33/L4: 1.00]\newline $e_5$, actor, Jonathan\_Pryce\newline Jonathan\_Pryce, film, $e_5$\newline Jonathan\_Pryce, film, $e_4$\newline $e_3$, actor, Johnny\_Depp \\
\bottomrule
\end{tabular}

\vspace{0.2cm}
\caption{Comparison of explanations generated by three competent methods for four representative examples. Each cell contains the $\delta \text{MRR}$ (the drop in prediction accuracy after removing the selected facts) in the first row, followed by the explanation sets generated by each model. For clarity, some entities are represented by abbreviations due to their lengthy names: 
$e_0$ refers to \texttt{Primetime\_Emmy\_Award\_for\_Outstanding\_Supporting\_Actress},
$e_1$ to \texttt{Frances\_McDormand},
$e_2$ to \texttt{1960\_Summer\_Olympics}, 
$e_3$ to \texttt{Pirates\_of\_the\_Caribbean:\_At\_World's\_End}, 
$e_4$ to \texttt{Pirates\_of\_the\_Caribbean:\_Dead\_Man's\_Chest}, and
$e_5$ to \texttt{Pirates\_of\_the\_Caribbean:\_The\_Curse\_of\_the\_Black\_Pearl}.}
\label{tab:example}
\end{table*}



The table~\ref{tab:example} presents four representative examples, comparing explanations generated by five competent models: Kelpie(L1), KGEAttack, eXpath(L1), Kelpie, and eXpath. The first three systems generate explanations of length 1, while the latter two systems produce explanations of length $\leq 4$. To simplify presentation, some entities are abbreviated, with their full names listed in the caption.

The first example highlights the strength of KGEAttack and eXpath(L1), both of which provide identical and highly effective explanations (head/tail rank drops from $1/1$ to $6/106$). Both systems leverage a compelling CP rule: \texttt{award\_nominee $\leftarrow$ award' [HC=0.816, SC=0.815, supp=9930]}, a clear and intuitive rule linking \texttt{award\_nominee} and \texttt{award} as inverse relations. By contrast, Kelpie’s relevance-based approach yields weaker results despite using four facts, underscoring its limitations when compared to high-quality, rule-based systems.

The second example reverses the trend, showing Kelpie(L1) outperforming KGEAttack. KGEAttack provides an intuitive single-hop rule: \texttt{country(X, Japan) $\leftarrow$ films\_in\_this\_genre(Anime, X) [SC=0.846]}, suggesting that a film in the Anime genre is likely associated with Japan. eXpath, however, outperforms both by presenting a richer explanation that combines multiple rules:
\begin{itemize}
    \item \texttt{Uc: country(X, Japan) $\leftarrow$ language(X, Japanese) [0.669]}
    \item \texttt{CP: country $\leftarrow$ language, language', country [0.072]}
    \item \texttt{CP: country $\leftarrow$ language, language', nationality [0.064]}
\end{itemize}
These three rules are representative of 20 length-3 CP rules identified by eXpath, each with a low SC but collectively yielding a confidence degree exceeding $0.9$. This result demonstrates that relying solely on individual or simple rules, as KGEAttack does, risks overlooking valuable signals in the data. Kelpie, while also producing effective explanations, relies heavily on empirical signals from model fine-tuning and lacks rule-based clarity. Interestingly, Kelpie’s performance here declines compared to Kelpie(L1), illustrating that larger explanation sets do not always enhance effectiveness. Removing too many facts without rule-based support may fail to degrade model predictions effectively, exposing the limitations of Kelpie’s purely empirical approach.

\begin{figure*}[t]
\includegraphics[width=\textwidth]{pic/exampleV4.png}
\caption{To explain the fact $\langle$Pirates\_of\_the\_Caribbean:\_At\_World’s\_End ($e_3$), actor, Jonathan\_Pryce$\rangle$ predicted by LP models (ComplEx), eXpath identifies the 3-hop subgraph around the head and tail entities, filters irrelevant facts, and extracts key rules. The right panel compares the sets of facts provided by Kelpie, KGEAttack, and eXpath. The red line represents the predicted fact, blue lines denote the explanatory facts extracted by each method, and gray lines indicate the paths formed by these facts.}
\label{example}
\end{figure*}


In the third and fourth examples, KGEAttack and Kelpie fail to produce effective explanations, while eXpath delivers highly effective results. Compared to eXpath(L1), eXpath(L4) consistently provides more impactful explanations, with higher $\delta \text{MRR}$ values. This highlights the importance of combining multiple facts for explanations, especially in dense datasets like \texttt{FB15k} and \texttt{FB15k-237}, where removing a single fact is often insufficient.

The fourth example presents an intriguing case involving the prediction $\langle e_3, actor, Jonathan\_Pryce\rangle$. Figure~\ref{example} (a) depicts the 3-hop subgraph of the KG surrounding the head and tail entities, showing the dense connections and relations that complicate the explanation process. Figure~\ref{example} (b) displays key rules with $SC > 0.05$ identified by eXpath for this example, while Figures~\ref{example} (c), (d), and (e) compare the sets of explanatory facts provided by Kelpie, KGEAttack, and eXpath, respectively. Kelpie and eXpath both offer explanations combining four facts, with single-fact versions highlighted in bold. Notably, eXpath(L4) delivers the most effective explanation, achieving nearly perfect attack effectiveness ($\delta \text{MRR}$ approaching $1$), while Kelpie(L4) also performs well ($\delta \text{MRR} = 0.58$). In contrast, explanations from KGEAttack and Kelpie(L1) are largely ineffective.

Kelpie provides fact-based explanations but does not justify why these facts support the prediction. Only one fact, $\langle e_4, sequel, e_3\rangle$, lies on a critical path; the remaining facts are not directly relevant. Moreover, removing this single fact leaves $\langle e_3, prequel, e_4\rangle$ intact as a reverse relation, undermining the explanation's validity. KGEAttack proposes a single attacking fact, $\langle e_3, prequel, e_4\rangle$, along with the rule $actor(X, Y) \leftarrow prequel(X, A), film(Y, A)$ [SC=0.37, supp=244]. While this 2-hop CP rule is intuitive, it fails for the same reason as Kelpie: reverse relations preserve the prediction, rendering the explanation insufficient.

In contrast, eXpath provides path-based explanations, combining selected facts with supporting rules. For instance, the highest-scoring fact, $\langle e_5, actor, Jonathan\_Pryce\rangle$, satisfies the following rules, among others:

\begin{itemize}
    \item \texttt{Uc: actor($e_3$, Y) $\leftarrow$ actor($e_5$, Y) [0.5]}
    \item \texttt{CP: actor $\leftarrow$ actor, award\_winner', actor [0.06]}
    \item \texttt{CP: actor $\leftarrow$ film', award\_winner', actor [0.05]}
    \item \texttt{CP: actor $\leftarrow$ film', honored\_for, actor [0.05]}
\end{itemize}

These rules, along with over 30 additional CP rules, collectively contribute to a cumulative score exceeding 0.5. Unlike KGEAttack, which focuses only on 2-hop CP rules, eXpath incorporates longer, more complex rules that capture additional signals in the data, albeit at the cost of reduced simplicity. As shown in Figure~\ref{example} (b), eXpath's explanations comprehensively cover all critical paths from $e_3$ to Jonathan Pryce, enabling a near-perfect explanation for the prediction.

Another notable observation is that most facts selected by eXpath relate to the tail entity rather than the head entity. As shown in Figure~\ref{example} (a), the head entity ($e_3$) is associated with $96$ triples, while the tail entity (Jonathan Pryce) has only $32$, making the tail relations sparser and more critical for the prediction. By considering the frequency of facts in both head and tail relations, eXpath prioritizes tail-related facts, leading to more effective explanations. In contrast, Kelpie relies primarily on head entity features, often falling into local optima and missing the broader context. Meanwhile, KGEAttack randomly selects from the rules it satisfies, resulting in explanations with high variability and limited reliability.

The case studies demonstrate the superiority of eXpath in generating semantically rich and effective explanations. By leveraging comprehensive rule-based reasoning and combining multiple facts, eXpath achieves an optimal balance of interpretability and explanatory power, consistently outperforming alternative methods.

